Experimental implementation of an emission-aware prosumer with online flexibility quantification and provision

Active building energy management holds potential to reduce global energy-related emissions and support flexible operations of future low-carbon systems. This requires to integrate diverse objectives and engage multiple stakeholders. However, there remains a gap in comprehensive field insights into emission reduction, flexibility provision, and user impacts. This study examined how a real occupied building, with all its energy assets, could function as an emission-aware flexible prosumer. An existing building energy management system was enhanced by integrating a model predictive control strategy. The enhanced setup minimized the equivalent carbon emission due to electricity imports and provided flexibility to the energy system. The experimental results indicated an emission reduction of 12.5% compared to a rule-based controller that maximized PV self-consumption. In addition, a minimal flexibility provision experiment was demonstrated with a locally emulated distribution system operator. The results suggested that flexibility was provided without the risk of rebound effects. This is due to the flexibility envelope that was self-reported in advance. The study concluded by highlighting technical challenges in realizing emission reduction and flexibility in practice.

==> sections/append_A.tex <==
\section*{Appendix A}
The mentioned works and the current study are further compared and summarized in \autoref{Table:comparison} with respect to the main focus, testbed, resources and whether flexibility is quantified online for real-time control. 

\begin{table}[!htbp]
    \centering
    \caption{Comparison of relevant research works.}\label{Table:comparison}
    \resizebox{\textwidth}{!}{%
\begin{tabular}{|p{1.2cm}|p{6.5cm}|p{5cm}|p{4cm}|l|}
\hline
Ref                                & Main focus                                                               & Testbed                              & Resources            & Flexibility \\ \hline
\cite{sturzenegger2015model}       & Economic MPC and cost benefit analysis       & Occupied office building & HVAC, Blind          & -           \\ \hline
\cite{vrettos2016experimental}     & Frequency regulation service                             & Two experimental rooms               & HVAC                 & -           \\ \hline
\cite{gorecki2017experimental}     & Frequency regulation service                                   & Five-room office building           & HVAC                 & -           \\ \hline
\cite{ruano2016imbpc}              & Economic MPC                                                             & Three lecture rooms                 & HVAC                 & -           \\ \hline
% \cite{yu2017model}                 & Energy-efficient MPC                                                     & Wooden chamber                    & HVAC                 & -           \\ \hline
\cite{viot2018model}               & Energy-efficient MPC                                                     & Experimental building               & HVAC                 & -           \\ \hline
\cite{joe2019model}                & Economic and energy-efficient MPC                                        & Three open-plan offices       & HVAC                 & -           \\ \hline
\cite{bolzoni2021model}            & Energy-efficient and emission-aware MPC                          & Battery and RTDS                    & HVAC and Battery        & -           \\ \hline
\cite{fiorentini2017hybrid}        & Multimode HVAC system                                            & Solar Decathlon house             & HVAC and PCM            & -           \\ \hline
% \cite{sangi2019real}               & An exergy-based MPC strategy                                             & Office building                   & HVAC                 & -           \\ \hline
\cite{bunning2020experimental}\cite{bunning2020input}     & Data predictive control                  & Two occupied rooms                    & HVAC                 & -           \\ \hline
\cite{jain2020neuropt}             & Data-driven energy-efficient MPC                                    & Two-story building                   & HVAC                 & -           \\ \hline
\cite{yang2020model}\cite{yang2021experiment}          & Machine learning-based MPC                                   & Office and lecture theater          & HVAC                 & -           \\ \hline
\cite{heinrich2020ecogrid}         & Flexibility market  & 121 households   &  HVAC            & Offline     \\ \hline
\cite{bernstein2015composable}     & Composable smart grid control & Campus building & Generic & Online \\
\hline
\cite{Chen2020258}                 & Aggregate power flexibility  & Simulation   & Generic     & Online      \\ \hline
\cite{munankarmi2020quantification} & Power flexibility band    & Simulated residential   &  HVAC, DHW, PV and battery    & Online      \\ \hline
\cite{kathirgamanathan2020towards} & Flexibility characterization     & Simulated commercial and residential buildings   & HVAC                 & Offline     \\ \hline
\cite{de2016quantification}        & Flexibility characterization           & Simulated office building   &  HVAC   & Online      \\ \hline
\cite{maasoumy2014model}           & Flexibility quantification and provision     & Simulated campus building   & HVAC                 & Online      \\ \hline
\cite{d2015demand}                 & Flexibility potential quantification     & 186 households                 & Wet appliances, DHW buffers and EV                   & Offline     \\ \hline
\cite{gasser2021predictive}        & MPC applications and flexibility quantification  & Simulated residential building   & HVAC, DHW and EV  & Online      \\ \hline
This paper                         & Emission-aware MPC, flexibility quantification and provision & Occupied three-room flat            & HVAC, DHW, EV and battery & Online      \\ \hline
\end{tabular}
    }
\end{table}
